A3: Assisting Android API Migrations Using Code Examples

The fast-paced evolution of Android APIs has posed a challenging task for Android app developers. To leverage Android's frequently released APIs, developers must often spend considerable effort on API migrations. Prior research and Android official documentation typically provide enough information to guide developers in identifying the API calls that must be migrated and the corresponding API calls in an updated version of Android (what to migrate). However, API migration remains a challenging task since developers lack the knowledge of how to migrate the API calls. There exist code examples, such as Google Samples, that illustrate the usage of APIs. We posit that by analyzing the changes of API usage in code examples, we can learn API migration patterns to assist developers with API Migrations. In this paper, we propose an approach that learns API migration patterns from code examples, applies these patterns to the source code of Android apps for API migration, and presents the results to users as potential migration solutions. To evaluate our approach, we migrate API calls in open source Android apps by learning API migration patterns from code examples. We find that our approach can successfully learn API migration patterns and provide API migration assistance in 71 out of 80 cases. Our approach can either migrate API calls with little to no extra modifications needed or provide guidance to assist with the migrations. Through a user study, we find that adopting our approach can reduce the time spent on migrating APIs, on average, by 29%. Moreover, our interviews with app developers highlight the benefits of our approach when seeking API migrations. Our approach demonstrates the value of leveraging the knowledge contained in software repositories to facilitate API migrations.

==> case.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=1\textwidth]{pictures/Stuff_good.png}%
\label{method}
\caption{Link Extraction Methodology}
\label{fig_methodology}
\end{figure*}

We based our study on previous research in framework migration suggestions \cite{1_dagenaisrobillard_2008,Robbes:2011:SRE:1985793.1985940,Cossette:2012:SGT:2393596.2393661,apiwattanapong_orso_harrold_2006,wang_many_to_many_map}. Motivated by the example presented in section \ref{example} we obtain and use information in a version control repository to produce links between similar and replacement API methods.
\par

Creating and following method links in a large API requires a thorough understanding of the API. Developers can sometimes substitute repository information by using their experience and intuition. However, attempting to automate the creation of links can only rely on data. Therefore, it is important to gather and process all information available with as little waste as possible. This includes internal documentation (JavaDoc), commit messages, and source code artifacts.

We decided to use the Android API as the primary target of our API evolution mapping study. This decision was based on the popularity of Android devices, the popularity of the API with app developers, and the 25 API migrations available as of this reports submission.

We extracted method uses from 415 open source Android applications available on FDroid \cite{f-droid}. We used these projects to determine removed method usage of the Android API. We also used the FDroid projects as a sample of the distribution of Android API version usage. Using this sample distribution, we chose which API versions we would chose to use as experimental data for migration suggestions.

We manually obtained official migration methods for all removed methods of our target API version. The data was manually extracted from the official Android documentation and framework repository \cite{android_developers_index, android_framework_git}. This data was used to determine whether our suggestions provided correct answers to link removed methods to their replacements.

We compared our suggestion results to FDroid projects method use. This was done in order to determine how often suggestions could be useful to the Fdroid app developers when migrating their apps.

Finally, we manually attempted migrations of three FDroid apps, from a target Android API 23 to API 24. This was done as a further evaluation on how suggestions could be used to migrate these apps to more recent versions of the Android API.

\subsection{Studied Systems}

Large APIs provide many opportunities for method removal and migration when a new version is released. With 26 releases, the Android API provides ample removals and changes to examine over the lifetime of the project. With over 2.2 million applications \cite{12_app} using the API, and over 1.5 million daily Android device activations  \cite{13_android} we can rest assured that the API has a sizable user base. Most of the applications are proprietary and do not grant access to their source code. Therefore, it is difficult to determine their use of the API. Consequently, we had to obtain a sample of Android projects that would provide their source code.

FDroid is a catalog of free and open source applications for the Android platform. FDroid provides both a web interface and an Android application to obtain the projects presented in their catalog. Most of the FDroid apps provide their source code through Github, an online source code repository. We targeted all FDroid applications that stored their source code on Github. This allowed us to obtain 415 different Android applications, with a median of 6 versions per application \ref{fig_Fdroid_Box_plot}. These projects were used to determine which methods are consumed by app developers. For each project, we determined API method use and the targeted Android API version. From this information, we were able to determine which methods would need to be migrated in order to increase the targeted API version.

\begin{figure}[!t]
\includegraphics[width=\columnwidth]{pictures/Target_SKD_Requirements_in_FDroid_Apps.png}
\centering
\caption{Target SDK Requirements in FDroid Apps}
\label{fig_Fdroid_targets}
\end{figure}

==> discussion.tex <==
discussion
